Dissecting Generation Modes for Abstractive Summarization Models via Ablation and Attribution

Despite the prominence of neural abstractive summarization models, we know little about how they actually form summaries and how to understand where their decisions come from. We propose a two-step method to interpret summarization model decisions. We first analyze the model's behavior by ablating the full model to categorize each decoder decision into one of several generation modes: roughly, is the model behaving like a language model, is it relying heavily on the input, or is it somewhere in between? After isolating decisions that do depend on the input, we explore interpreting these decisions using several different attribution methods. We compare these techniques based on their ability to select content and reconstruct the model's predicted token from perturbations of the input, thus revealing whether highlighted attributions are truly important for the generation of the next token. While this machinery can be broadly useful even beyond summarization, we specifically demonstrate its capability to identify phrases the summarization model has memorized and determine where in the training pipeline this memorization happened, as well as study complex generation phenomena like sentence fusion on a per-instance basis.

==> tab_cases_full.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[]
\centering
\small
\begin{tabular}{@{}ccp{13cm}@{}} \toprule
\multicolumn{3}{c}{Example} \\
Index &
  Prob &
  \multicolumn{1}{c}{Content} \\
0: &
  0.00 &
  Atherton, 28, has won all seven races this season and 13 in a row, a run stretching back to 2015. \\
1: &
  0.09 &
  The world champion had already sealed the 2016 World Cup crown in Canada last month but won in Andorra on Saturday to end the World Cup season unbeaten. \\
2: &
  0.01 &
  She has now won five overall World Cup titles in downhill. \\
3: &
  0.07 &
  Wales' Manon Carpenter completed a British one-two in the overall standings, finishing 560 points behind Atherton. \\
4: &
  0.16 &
  Trek Factory Racing's Atherton won the final race by 6.5 seconds ahead of Australian Tracey Hannah and Myriam Nicole of France. \\ \midrule
Comb &
  Prob &
  \multicolumn{1}{c}{Predict Summary} \\
(1, 4) &
  0.71 &
  Britain's Laura Atherton has won the UCI \\ \bottomrule \toprule
\multicolumn{3}{c}{Example} \\
Index &
  Prob &
  \multicolumn{1}{c}{Content} \\
0 &
  0.01 &
  Dujardin, 30, and Valegro won individual and team dressage gold for Britain at London 2012 and have since won World and European titles. \\
1 &
  0.00 &
  But, she says, the Olympics in Brazil next summer will be the horse's last. \\
2 &
  0.01 &
  "This will be Valegro's retirement after Rio so I want to go out there and want to enjoy every last minute," Dujardin told BBC Points West. \\
3 &
  0.00 &
  Media playback is not supported on this device \\
4 &
  0.00 &
  Dujardin partnered Valegro to victory in London as the two performed to movie themes including The Great Escape and Live And Let Die. \\ \midrule
Comb &
  Prob &
  \multicolumn{1}{c}{Predict Summary} \\
(0, 1) &
  0.63 &
  Olympic dressage champion Charlotte Dujardin says she will retire \\ \bottomrule \toprule
\multicolumn{3}{c}{Example} \\
Index &
  Prob &
  \multicolumn{1}{c}{Content} \\
0 &
  0.00 &
  In a letter sent to the court that convicted him, he says it would be easier - and less expensive - for his family to visit him in Africa. \\
1 &
  0.00 &
  He also said he feared being attacked in a British prison. \\
2 &
  0.33 &
  Taylor was convicted of aiding rebels who committed atrocities in Sierra Leone during its civil war. \\
3 &
  0.00 &
  Last week, a UK minister confirmed that Taylor would be transferred to a British prison. \\
4 &
  0.00 &
  He was convicted by the UN-backed Special Court for Sierra Leone (SCSL), but his trial was held in The Hague in case it sparked renewed unrest in West Africa. \\
5 &
  0.00 &
  The Netherlands only agreed to host the trial if he was imprisoned elsewhere. \\
6 &
  0.00 &
  In a letter seen by the BBC, Taylor wrote: \\
7 &
  0.00 &
  "My position is that serving my sentence in Rwanda, in my home continent of Africa, would be substantially more humane not only on my own account, but also on account of the impact on my family." \\
8 &
  0.00 &
  He noted that the court's statutes said access for prisoners' relatives should be taken into account when deciding where they should serve their sentence. \\
9 &
  0.27 &
  • 1989: Launches rebellion in Liberia \\
10 &
  0.00 &
  • 1991: RUF rebellion starts in Sierra Leone \\ \midrule
Comb &
  Prob &
  \multicolumn{1}{c}{Predict Summary} \\
(6, 9) &
  0.93 &
  Liberia's former President Charles Taylor has said he will \\ \bottomrule
\end{tabular}
\caption{}
\label{tab:cases}
\end{table*}

==> tab_two_stage.tex <==
\begin{table}[h]
\centering
\footnotesize
\begin{tabular}{ccccccc} \toprule
                     & \multicolumn{6}{c}{\textsc{Disp} $\downarrow$}                                \\
                     & 0                     & 1    & 2    & 4    & 8    & $-\Delta$ \\ \midrule
S + Occl    & \multirow{4}{*}{4.61} & 4.27 & 3.93 & 3.31 & 2.71 & 0.84     \\
S + Attn  &                       & 3.85 & 3.63 & 3.15 & 2.68 & \textbf{1.03}     \\
S + InpGrad &                       & 4.21 & 3.98 & 3.63 & 3.23 & 0.68     \\
S + IntGrad &                       & 4.46 & 4.30 & 4.10 & 3.81 & 0.35    \\ \bottomrule
\end{tabular}
\caption{Token-level evaluation for content attribution methods. S+Attention works the best and S+IntGrad performs worst. }
\label{tab:two-stage}
\end{table}
